Textbooks Are All You Need

We introduce phi-1, a new large language model for code, with significantly smaller size than competing models: phi-1 is a Transformer-based model with 1.3B parameters, trained for 4 days on 8 A100s, using a selection of ``textbook quality" data from the web (6B tokens) and synthetically generated textbooks and exercises with GPT-3.5 (1B tokens). Despite this small scale, phi-1 attains pass@1 accuracy 50.6% on HumanEval and 55.5% on MBPP. It also displays surprising emergent properties compared to phi-1-base, our model before our finetuning stage on a dataset of coding exercises, and phi-1-small, a smaller model with 350M parameters trained with the same pipeline as phi-1 that still achieves 45% on HumanEval.

==> tikzlibraryshapes.emoticon.code.tex <==
%
%
%
\pgfdeclareshape{emoticon happy}
{
  \inheritsavedanchors[from=circle] 
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritbackgroundpath[from=circle]
  %
  %
  %
  \inheritbackgroundpath[from=circle]
  \beforebackgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \color{black}
    \pgfpathellipse{\pgfqpoint{.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
    \pgfpathellipse{\pgfqpoint{-.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
                          \pgfusepath{stroke}%
\begingroup
\pgfsetlinewidth{0.4pt}%
\pgflowlevelsynccm    
       \pgfpathmoveto{\pgfqpoint{-.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}%
      \pgfpatharc{-135}{-45}{.5\pgfutil@tempdima and .5\pgfutil@tempdima}%
      \pgfusepath{stroke}%
\endgroup    
  }} 

  \pgfdeclareshape{emoticon sad}
{
  \inheritsavedanchors[from=circle] 
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritbackgroundpath[from=circle]
  %
  %
  %
  \inheritbackgroundpath[from=circle]
  \beforebackgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \color{black}
    \pgfpathellipse{\pgfqpoint{.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
    \pgfpathellipse{\pgfqpoint{-.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
                          \pgfusepath{stroke}%
\begingroup
\pgfsetlinewidth{0.4pt}%
\pgflowlevelsynccm    
      \pgfpathmoveto{\pgfqpoint{-.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}%
 \pgfpathcurveto{\pgfqpoint{-.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}
                {\pgfpoint{0pt}{-.153\pgfutil@tempdima}}
                {\pgfqpoint{.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}
      \pgfusepath{stroke}%
\endgroup    
  }}  

    \pgfdeclareshape{emoticon straight face}
{
  \inheritsavedanchors[from=circle] 
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritbackgroundpath[from=circle]
  %
  %
  %
  \inheritbackgroundpath[from=circle]
  \beforebackgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \color{black}
    \pgfpathellipse{\pgfqpoint{.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
    \pgfpathellipse{\pgfqpoint{-.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
                    \pgfusepath{fill}%
                          \pgfusepath{stroke}%
\begingroup
  \pgfsetlinewidth{0.4pt}%
  \pgflowlevelsynccm    
  \pgfpathmoveto{\pgfqpoint{-.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}%
  \pgfpathlineto{\pgfqpoint{.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}
  \pgfusepath{stroke}%
\endgroup    
  }}  
      \pgfdeclareshape{emoticon wink}
{
  \inheritsavedanchors[from=circle] 
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritbackgroundpath[from=circle]
  %
  %
  %
  \inheritbackgroundpath[from=circle]
  \beforebackgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \color{black}
    \pgfpathmoveto{\pgfqpoint{-.40\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
    \pgfpathcurveto{\pgfqpoint{-.40\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                {\pgfqpoint{-.25\pgfutil@tempdima}{.10\pgfutil@tempdima}}%
                {\pgfqpoint{-.10\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
    \pgfpathellipse{\pgfqpoint{.25\pgfutil@tempdima}{.25\pgfutil@tempdima}}%
                   {\pgfqpoint{.1\pgfutil@tempdima}{0pt}}%
                   {\pgfqpoint{0pt}{.15\pgfutil@tempdima}}%
    \pgfusepath{fill}%
    \pgfusepath{stroke}%
\begingroup
   \pgfsetlinewidth{0.4pt}%
   \pgflowlevelsynccm    
   \pgfpathmoveto{\pgfqpoint{-.353\pgfutil@tempdima}{-.353\pgfutil@tempdima}}%
   \pgfpatharc{-135}{-45}{.5\pgfutil@tempdima and .5\pgfutil@tempdima}%
   \pgfusepath{stroke}%
\endgroup      
  }}%
\endinput
